A posteriori error estimates by weakly symmetric stress reconstruction for the Biot problem

A posteriori error estimates are constructed for the three-field variational formulation of the Biot problem involving the displacements, the total pressure and the fluid pressure. The discretization under focus is the H1({\Omega})-conforming Taylor-Hood finite element combination, consisting of polynomial degrees k + 1 for the displacements and the fluid pressure and k for the total pressure. An a posteriori error estimator is derived on the basis of H(div)-conforming reconstructions of the stress and flux approximations. The symmetry of the reconstructed stress is allowed to be satisfied only weakly. The reconstructions can be performed locally on a set of vertex patches and lead to a guaranteed upper bound for the error with a constant that depends only on local constants associated with the patches and thus on the shape regularity of the triangulation. Particular emphasis is given to nearly incompressible materials and the error estimates hold uniformly in the incompressible limit. Numerical results on the L-shaped domain confirm the theory and the suitable use of the error estimator in adaptive strategies.

==> old.tex <==
\section{Stress and Flux variables in the Biot Model}

on a reference configuration $\Omega\subset \R^2$
For $\bx \in \Omega$ and at a time $t$, the fluid pressure is denoted by $\phi(\bx,t)$ and the displacement of the solid by $\Disp(\bx,t)$. 


\fixme{In this section, we should emphase the importance of the auxiliary variables like stress and flux and their physical meanings!}
The classical Biot model of consolidation under our consideration describes a linearly elastic and porous structure with reference configuration $\Omega\subset \R^2$, which is saturated by a slightly compressible viscous fluid. For $\bx \in \Omega$ and at a time $t$, the fluid pressure is denoted by $\phi(\bx,t)$ and the displacement of the solid by $\Disp(\bx,t)$. 

$\Omega$ is assumed to be a an open, bounded, and connected domain with Lipschitz-continuous boundary $\Gamma$ divided in two disjoint nonempty subsets $\Gamma_u$ and $\Gamma_p$. On $\Gamma_u$, homogeneous displacement boundary conditions are imposed while surface traction forces are prescribed on $\Gamma_p$.
The equations for the quasi-static Biot model are given by 
\begin{subequations}\label{Biot}\begin{align}
\div \left(
	\sigmaexp{\Dispt}- \alpha \phi(t)  \bI
 \right)  = \bff(t) \\
 s_0 \difft \phi(t)+\alpha \div \difft \Dispt-\div(\kappa \nabla \phi(t)) = g(t)
\end{align}\end{subequations}
The analysis of numerical treatment can be reduced to stationary case \fixme{(this sentence needs to be rewriten in a more diplomatic way)}
\begin{subequations}\label{Biot_stationary}\begin{align}
\div \left(
	\sigmaexp{\Disp}- \alpha \phi  \bI
 \right)  = \bff \\
 s_0 \phi+\alpha \div  \Disp-\div(\kappa \nabla \phi) = g
\end{align}\end{subequations}
where for simplicity we did not change the definition of $\bff$ and $g$. Note that the first equation is the momentum equation and can be rewritten as 
\begin{align}
\div \left(
	\Stress(\Disp) - \alpha \phi  \bI
 \right)  = \bff
 \end{align}
 where $\Stress(\Disp) := \sigmaexp{\Disp}$ denotes the elastic stress or 
 \begin{align*}
\div 
	\TotalStress 
  = \bff \ ,
 \end{align*} 
 with the total stress tensor $\TotalStress = \TotalStressdef{}{}$. %expressing the fact that an increase in pore pressure induces a dilation of the matrix in response to the added stress.
  \fixme{point out the importance of Hdiv conformity for those variables. Conservation law. Surface tension forces of the solid structure}

\fixme{emphize the advantages of RT reconstructions and cite papers with AW reconstructions.}
\fixme{make clear that the motivation is two-folds: approximation in Hdiv and a posteriori}
For the fluid velocity, the Braess-Schöberl algorithm rom \cite{BraSch:08} reconstructing the conforming approximation of the solution of the Poisson equation in the Raviart-Thomas Finite element space can be used. A major advantage is that the reconstruction can be localised on the vertex-patches
\begin{equation}
  \omega_\nu := \bigcup \{ T \in \cT_h : \nu \mbox{ is a vertex of } T \} \: .
  \label{eq:vertex_patch}
\end{equation}
involving the partition of unity
\begin{equation}
  1 \equiv \sum_{\nu \in \mathcal V_h} \chi_\nu  ,
  \label{eq:partition_of_unity_1}
\end{equation}
and the localised broken Raviart-Thomas spaces
\begin{align}
RT^\Delta_\nu := \{ 
\bw_h
 \in  L^2(\omega_\nu)  : \left.
 \bw_h 
 \right|_T 
 \in RT_k (T), \bw_h \cdot \bn = 0 \} \ .
\end{align}
To a function $f \in L^2(\Omega)$ and a flux $\bw_h \in \mathbb P_k(\mathcal T_h)^2$ we denotes the Braess-Schöberl reconstruction of order $k$ by $\bw_h^R = \BR^k(f, \bw_h )$ the function 
$\bw_h^R \in RT^k(\mathcal T_h)$  with 
$\bw_h^R = \bw_h +\bw_h^{\Delta}$ and 
$\bw_h^{\Delta} = \sum_{\nu \in \mathcal V} \bw_{h,\nu}^{\Delta}$
and $\bw_{h,\nu}^{\Delta} \in DRT^\Delta(\omega_\nu)$ such that $\|\bw_{h,\nu}^{\Delta}\|$ is
minimized subject to the following constraints:
\begin{equation}
  \begin{split}
     \div \: {\bw_{h,\nu}^\Delta } 
    & = - \Pi^k_T \left( ({\bff} + \div \: \bw_h) \phi_\nu \right) \text{ on each }T\in \omega_\nu
   \\
     \llbracket \bw_{h,\nu}^\Delta \cdot \bn \rrbracket_S 
    & =  - \Pi^{k}_S  \left( \phi_\nu \llbracket 
    \bw_h \cdot \bn 
    \rrbracket_S \right) \text{ for each } S \text{ interior edge in } \omega_z \ .
  \end{split} 
  \label{eq:equilibration_conditions_local}
\end{equation}
To simplify the notation, we define
$\BR^k_\nu(f, \bw_h ) := \bw_{h,\nu}^\Delta$ 
\fixme{( Can i write this inverse mapping in an explicit way? )}
and for a tensor $\Stress = 
\left( \Stress_1 \ \Stress_2 \right)^\top \in RT^k(\mathcal T_h)^2$ and a vector-valued function $\bff = 
\left( f_1 \ f_2 \right)^\top \in L^2(\Omega)^2$ , the Braess-Schöberl construction $\BR^k(f, \bw_h )$ is defined elementwise:
\begin{align}
\BR^k(\bff, \Stress ) := 
\begin{pmatrix}
 \BR^k(f_1, \Stress_1 ) \\
 \BR^k(f_2, \Stress_2 )
\end{pmatrix}
\end{align}

For the purpose of the exposition, we recall the condition for existence and the properties of the Braess-Schöberl construction in the next theorem. 
\begin{thm}[Braess-Schöberl algorithm for Poisson equation, \cite{}]
Assume that $f \in \mathbb P _{k-1}(\mathcal T_h)$ and $\tilde p_h \in \mathcal P _k(\mathcal T_h) \cap H_{\Gamma_u}^1(\Omega) $ is the discrete solution of the Poisson equation, i.e.
\begin{align}
\left ( \nabla \tilde p_h, \nabla q \right) = \left ( f,  q \right) \quad \forall q \in \mathcal P _k(\mathcal T_h) \cap H_{\Gamma_u}^1(\Omega)  \ .
\end{align}
The Braess-Schöberl reconstruction $\bw_h^R = \Psi(f, \bw_h) \in RT{k-1}(\tri)$ exists and satisfies
\begin{subequations}
\begin{align}
\div \bw_h^R &= f \\
\norm{\nabla (\tilde p-\tilde p_h)} &\leq \norm{\bw_h^R-\bw_h} \\
\fixme{\text{insert other properties i may need}}
\end{align}
\end{subequations}
where $\tilde p$ denotes the exact solution of the Poisson equation $\div \nabla \tilde p = - f$.
\end{thm}
Note that a crucial condition for this theorem to hold is the compatibility condition
\begin{align*}
\fixme{\text{insert compatibility condition}}
\end{align*} 
In order to apply this construction to the Biot problem, we shift the first two terms of \eqref{twofields_h2} to the right side, following \cite{Riedelbeck} and define $\tilde g = g- s_0 p_h-\alpha \div \Disp $.


For the reconstruction of the stress, \cite{BerKobMolSta:19} showed that the symmetry has to be taken into account. The authors considered a the displacement pressure formulation but we will show that the reconstruction can be applied to the standard conforming displacement formulation of linear elasticity. In fact, the construction of the authors is equivalent to a minimization in the divergence free Raviart-Thomas space of order $k$
 \begin{align}
RT_k^\times(\omega_\nu) = 
\left\{
\bw \in RT_k(\omega_\nu) \ : \ \div \bw = 0
 \right\} \ ,
\end{align} 
where the difference between the reconstructed stress and the stress computed from the variational formulation belong to the 
weakly symmetric broken Raviart-Thomas space of order $k$
 \begin{align*}
DRT_k^{ws}(\omega_\nu) = 
\left\{
\begin{pmatrix}
 \tau_1
 \\ 
 \tau_2
 \end{pmatrix}
 \in (DRT_k(\omega_\nu))^2 \ : 
  \right.%&
 %\\ & 
 \left.
\left(
\tau_1 \cdot 
 \begin{pmatrix} 1 \\ 0 
 \end{pmatrix}
 -
  \tau_2 \cdot 
 \begin{pmatrix} 0 \\ 1  
 \end{pmatrix}, \chi
 \right)_{\omega_\nu}
  = 0 
  \text{ for all }\chi \in \mathcal P^k(\mathcal T_h)
 \right\} \ .
\end{align*}
%For $\Stress_\nu \in DRT_k(\omega_\nu)^2$, let $\symcomp{\nu}{ \Stress_\nu}$ denotes the minimisation of the norm under the symmetry constraint:
%\begin{align}
%\symcomp{\nu}{ \Stress_\nu}
% = \argmin_{
% \underset{s.t.\ \Stress_\nu + \Stress \in RT_k^{ws}(\omega_\nu) }{
% \Stress \in RT_k^\times(\omega_\nu)^2}
% } \|\Stress_\nu + \Stress \|
%\end{align}
For $\Stress_h \in DRT_k(\tri)^2$, let $\symcomp{\nu}{ \Stress_\nu}$ denotes the minimisation of the norm under the symmetry constraint:
\begin{align}
\symcomp{\nu}{ \Stress_h}
 =  \argmin_{
 \underset{s.t.\ \Stress_h + \Stress \in DRT_k^{ws}(\omega_\nu) }{
 \Stress \in RT_k^\times(\omega_\nu)^2}
 } \|\Stress_h + \Stress \|
\end{align}
Further notation:
\begin{align}
\symcomp{}{\Stress_h} := \sum\limits_{\nu\in \nodes} \symcomp{\nu}{ \Stress_h} \text{ and }\widetilde \Pi(\Stress_h):=\Stress_h + \symcomp{}{\Stress_h} 
\end{align}
\fixme{this is a projection on a $\sigma$-dependant space, maybe the notation should be changed.}

\begin{thm}
Assume that ${\bff} \in (\mathbb P _k(\mathcal T_h))^2$. Let $\tilde \Disp_h \in \HDisph$ be the discrete solution of the variational formulation
\begin{align} \label{standard_conforming_elasticity}
 \left( \Stress({\tilde\Disp_h}), \symgrad{\DispTest}{} \right) = \left( {\bff} , \DispTest \right)
 \quad \forall \DispTest \in \HDisph \ .
\end{align}
Then, the weakly symmetric reconstruction 
$\Stress_h^R({\tilde\Disp_h}) =
 \widetilde \Pi \left(
\BR^k ({\bff}, \Stress({\tilde\Disp_h})) \right)		$
exists and satisfies
\begin{subequations}
\begin{align}
\div \Stress_h^R({\tilde\Disp_h}) = {\bff}\\
\fixme{\text{In particular here we should list all the properties for elasticity}}
\end{align}
\end{subequations}
\end{thm}
\begin{proof}
\fixme{...}
\end{proof}



\begin{remark}
enough degrees of freedom since the Braess-Schöberl reconstruction already satisfies the weekly symmetric condition.
\end{remark}

\mynote{
Set $\Stress_{h,z}^\Delta = \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta$
\begin{align*}
( \div \: \Stress_{h,z}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}
    & = - ( ( \bff + \div \: \Stress_h ) \phi_z ,
    \bz_{h,z}  )_{\omega_z,h}
    \\
    \langle \llbracket \Stress_{h,z}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            = & - \langle \llbracket \Stress_h \cdot \bn \rrbracket_S \, \phi_z , \zeta \rangle_S
   \\
    (
     \Stress_{h,z}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & = 0
\end{align*}
Since $\Stress_{h,z,BR}^\Delta$ satisfies the first two equations
it remains\\
$( \div \: (\Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta) , 
\bz_{h,z} )_{\omega_z^\ast,h}
     = - ( ( \bff + \div \: \Stress_h ) \phi_z ,
    \bz_{h,z}  )_{\omega_z,h}$\\
    i.e.
    $( \div \: 
\Stress_{h,z,AS}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}  = 0$\\
und $\langle \llbracket \Stress_{h,z,AS}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            =  0$
       also minimize $\| \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta \|$
       \begin{align*}
( \div \: \Stress_{h,z,AS}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}
    & =0
    \\
    \langle \llbracket \Stress_{h,z}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            = & 0
   \\
    (
     \Stress_{h,z,AS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & =  -\Stress_{h,z,BS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} 
\end{align*}
Find $\Stress_{h,z,AS}^\Delta$ in RTdivfree, such that 
$\| \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta \|$ is minimum, and
       \begin{align*}
    (
     \Stress_{h,z,AS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & =  -(\Stress_{h,z,BS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} 
\end{align*}
}


Energy-norm:
\begin{align}
\energy{(\Disp,p)}^2 = \energyds{2}{\Disp}{p}
\end{align}
Error estimator
\begin{align}
\eta(\Disp_h,p_h) = \left( \norm{(\Stress_h^R}^2
+
\norm{\kappa \bw_h^R}^2
\right)^{\frac 1 2}
\end{align}
more general version of Vertex-patch estimate.
\begin{lem}
\label{vertex-patch-all}
Let $\Stress_h \in DRT_k(\tri) $. 
If it exists, the reconstruction 
$\widetilde \Pi  {\BR^k({\bff}, \Stress_h ) }$ satisfies 
\begin{align}
 (\as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },{\DispTest}{})
 \leq  C_K \| \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h )  }\|
 \norm{\symgrad{\DispTest}{}}
\end{align}
for any $\DispTest  \in \HDisp$, where $C_K$ depends only on the shape regularity of the triangulation $\tri$.
\end{lem}
\begin{proof}
For any $\nu \in \nodes$, the existence of $ \widetilde \Pi  {\BR^k({\bff}, \Stress_h )} $ implies that we can find $\symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )}}
 \in RT_k^\times(\omega_\nu)^2$ with 
\begin{align*}
{\BR^k({\bff}, \Stress_h )}  
+ \symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )} } \in DRT_k^{ws}(\omega_\nu) 
\end{align*}
such that for all $\chi \in \mathcal P^k(\tri)$
\begin{align*}
\left(\as
\widetilde \Pi  {\BR^k({\bff}, \Stress_h )} 
, \chi 
\right) 
=
 \sum\limits_{\nu \in \mathcal V_h}
\left(\as
{\BR^k({\bff}, \Stress_h )}  
+ \symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )} }
, \chi 
\right)_{\omega_\nu}
= 0
\end{align*}
 holds. In particular, for any rigid body motion $\brho$
 \begin{align*}
\left(\as
\widetilde \Pi  {\BR^k({\bff}, \Stress_h )} 
, \nabla\brho
\right) 
= 0
\end{align*}
 such that we can use the Korn inequality to obtain
\begin{align*}
 (\as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },{\DispTest}{})
 &= 
  \left(
  \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },
{\DispTest-\brho}
\right) \leq C_K 
\| \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h )}\| 
\norm{\symgrad{\DispTest}{}}
\end{align*}
involving a local Korn constant $C_K$ depending only on the shape triangularity of the triangulation $\tri$.
%  \begin{equation}
%    \begin{split}
%      | ( \bas \: \bsigma_h^R , \bnabla (\bu - \bu_h) ) |
%      & = | ( \bas \: \bsigma_h^R , \sum_{z \in \cV_h} \left( \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \right) \phi_z ) | \\
%      & = \left| \sum_{z \in \cV_h} ( \bas \: \bsigma_h^R ,
%      \left( \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \right) \phi_z )_{\omega_z} \right| \\
%      & = \left| \sum_{z \in \cV_h} ( (\bas \: \bsigma_h^R) \phi_z , \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) )_{\omega_z} \right| \\
%      & \leq \sum_{z \in \cV_h} \| (\bas \: \bsigma_h^R) \phi_z \|_{\omega_z}
%      \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z} \\
%      & \leq \sum_{z \in \cV_h} \| \bas \: \bsigma_h^R \|_{\omega_z} \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z} \: .
%    \end{split}
%    \label{eq:asym_partition}
%  \end{equation}
%  For all rigid body modes $\brho \in \bR\bM$, $\bnabla \brho = \bJ^d (\balpha_z)$ holds with some $\balpha_z \in \R^{d (d-1)/2}$
%  and therefore
%  \begin{equation}
%    \inf_{\balpha_z} \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z}
%    \leq \inf_{\brho \in \bR\bM} \| \bnabla (\bu - \bu_h - \brho) \|_{\omega_z}
%    \leq C_{K,z} \| \bepsilon (\bu - \bu_h) \|_{\omega_z}
%    \label{eq:Korn_average}
%  \end{equation}
\end{proof}


\section{Three field formulation}
$p := - \lambda \div \Disp + \alpha \phi$ introduced in  \cite{Lee} . 

$p_S = \lambda \div \Disp = \alpha \phi -p_T$

\begin{equation}
\begin{aligned}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \boldsymbol{H}_{0}^{1} \\
%
-\left(\div \Disp, q\right)
-\left(\lambda^{-1} p, q\right)
+\left(\alpha \lambda^{-1} \phi, q\right) 
&=0, & \forall \quad q \in L^{2} \\
%
\left(\alpha \lambda^{-1} p, \psi\right)-2\left(\alpha^{2} \lambda^{-1} \phi, \psi\right)-\left(\kappa \nabla \phi, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in H_{0}^{1} 
\end{aligned}\end{equation}

Our purpose is a robust a posteriori error estimate, when $\lambda$ tends to infinity.
Note that in the incompressible case, the equations are decoupled which reflect the physical process.
\begin{equation}
\label{Lee}
\begin{aligned}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \boldsymbol{H}_{0}^{1} \\
%
-\left(\div \Disp, q\right)
&=0, & \forall \quad q \in L^{2} \\
%
-\left(\kappa \nabla \phi, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in H_{0}^{1} 
\end{aligned}\end{equation}

\begin{equation}
\label{Lee_h}
\begin{aligned}
\symgrad{\Disp_h}{\DispTest} 
-\left(\div \DispTest, p_{T,h}\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \HDisph \\
%
-\left(\div \Disp, q\right)
&=0, & \forall \quad q \in \Hp \\
%
-\left(\kappa \nabla p_{F,h}, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in \HDisph 
\end{aligned}\end{equation}

We now return back to a general $\lambda$, possibliy infinity.
\begin{equation}
  \Stress (\Disp,p) = 2 \mu \symgrad{\Disp}{} + p\bI
  \label{eq:direct_stress}
\end{equation}
The approximation
\begin{equation}
  \Stress_h (\Disp_h,p_h) = 2 \mu \symgrad{\Disp_h}{} + p_{h} \bI
  \label{eq:direct_stress_processing}
\end{equation}

First line:
\begin{align*}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=
\symgrad{\Disp}{\DispTest} 
+\left(\div \DispTest,  p_S - \alpha \phi\right) \\&
=
\left(
\Stress(\Disp),
\symgrad{\DispTest}{} 
\right)
-\left(\div \DispTest,  \alpha \phi\right) 
\end{align*}

For the reconstruction of an $\Hdiv$-conforming stress tensor we use the main result from \cite{BB} about the weakly symmetric stress reconstruction of the displacement-pressure formulation. We recall this result here for the purpose of the exposition.
\begin{thm}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor arising from displacement-pressure formulation]
\label{thm-weaklystressreco}
 \fixme{Write it here, maybe in a more general way?}
\end{thm}

\begin{cor}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor for the three-field formulation of the Biot model]
 \fixme{...}
\end{cor}
\begin{proof}
\fixme{ compatibility condition}
\end{proof}

As for the two-fields formulation, we will reconstruct the total stress tensor. In this three fields formulation, the approximation of the stress tensor reads
\begin{align*}
\TotalStress_h = \TotalStressdef{\Disp_h,p_{S,h}}{p_{F,h}}
\end{align*}
From \eqref{} and \eqref{} we therefore obtain the equilibration condition 
 \begin{align*}
\div 
	\TotalStress 
  = \bff \ .
 \end{align*} 
 
\begin{thm}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor arising from displacement-pressure formulation]
 \fixme{Write it here, maybe in a more general way?}
\end{thm}
\begin{proof}
\fixme{ Use \ref{thm-weaklystressreco}}
\end{proof}

\begin{cor}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. $p_h$ is the discrete solution of the Poisson equation with right hand side $\tilde f =  {\Pi_k(g- s_0 p_h-\alpha \div \Disp_h )}$ and its Braess-Schöberl reconstruction $\bw_h^R$ 
exists and satisfies
\begin{equation}
  \begin{split}
     \div \: {\bw_{h}^R } 
    & =  {\Pi^{k-1}(g- s_0 \phi_h-\alpha \div \Disp_h )}  
  \end{split}
\end{equation}
\begin{align*}
\fixme{...}
\end{align*}
\end{cor}
\begin{proof}
The crucial compatibility condition holds, since $p_h$ is the solution of the Poisson equation with right hand side $f =  {\Pi_k(g- s_0 p_h-\alpha \div \Disp_h )}$.
\end{proof}
This leads to a $\Hdiv$ conforming reconstruction which can be used to evaluate the surface traction forces as illustrated in the numerical experiments in section \ref{sec-numerical-results}.

\begin{cor}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. The reconstruction 
\begin{align}
\Stress_h^R =\widetilde \Pi {\BR^k({\bff}-\nabla p_h, \Stress({\Disp_h})) }
\end{align}
exists and satisfies
\begin{subequations}
\begin{align}
\Stress_h^R &\in \bHdiv \\
\div\Stress_h^R &= \Pi^k \bff -\nabla p_h\\
\norm{\Stress - \Stress_h^R}_{\Gamma_u, div} &\leq h^k | \Stress|_{k+1} \fixme{\text{add oscillations and u,p norm?}}
\end{align}
\end{subequations}
\end{cor}
The reconstruction of $\Stress$ allows for the evaluation of the surface traction force, see {\fixme{example X}}. For the a posteriori error estimation however, it is necessary to consider the reconstruction of the total stress reconstruction, as presented in the following theorem.

\begin{thm}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. The reconstruction 
\begin{align}
\TotalStress_h^R 
=\widetilde \Pi{\BR^k_\nu({\bff}, \TotalStress_h ) }
\end{align}
exists and satisfies
\begin{align*}
\TotalStress_h^R \in (\bHdiv)^2\\
\div \TotalStress_h^R  = \Pi^k \bff \\
\end{align*} 
\end{thm}
\begin{proof}
The construction of $\TotalStress_h^R$ implies that
$\TotalStress_h^R = \TotalStress_h +\TotalStress_h^{\Delta}$ with
$\TotalStress_h^{\Delta} = \sum_{\nu \in \mathcal V} \TotalStress_{h,\nu}^{\Delta}$
and $\TotalStress_{h,\nu}^{\Delta} \in (DRT^\Delta(\omega_\nu))^2$ such that $\|\TotalStress_{h,\nu}^{\Delta}\|$ is
minimized subject to the following constraints:
\begin{equation}
  \begin{split}
     \div \: {\TotalStress_{h,\nu}^\Delta } 
    & = -  {\Pi^k \left(\phi_\nu\left(g- s_0 p_h-\alpha \div \Disp_h
    - \div \: \bpsi_h  \right)\right)} 
 \\
     \llbracket \bpsi_{h,\nu}^\Delta \cdot \bn \rrbracket_S 
    & =  - \Pi^{k}_S \left( \phi_\nu  \llbracket \bpsi_h \cdot \bn  \rrbracket_S\right) \text{ for each } S \text{ interior edge in } \omega_z
  \end{split}
\end{equation}
\end{proof}

\section{Compressible case and two-fields formulation}
The two-fields formulation \fixme{insert citations} seeks $(\Disp,p_F) \in \HDisp \times \Hp$ such that
\begin{subequations}\label{twofields}
\begin{align}
%(\sigmaexp{\Disp}- \alpha p_F  \bI,\nabla \DispTest)
(\symgrad{\Disp}{\DispTest})+(\lambda(\div \Disp) \bI- \alpha p_F  \bI,\nabla \DispTest)
  &=
( \bff,\DispTest) \quad \forall \DispTest \in \HDisp\\
 (s_0 p_F,q)+(\alpha \div \Disp, q)+(\kappa \nabla p_F,\nabla q) &= (g,q) \quad \forall q \in \Hp
\end{align}\end{subequations}
holds for all $(\DispTest,q) \in \HDisp \times \Hp$.
For the finite element approximation of the system \eqref{Biot_stationary}, the saddle-point problem \eqref{twofields} is solved in finite-element spaces. To this end, let $\mathcal T_h$ be a regular triangulation of the domain $\Omega$ where the diameter $\rho(T)$ of each element $T\in \mathcal T_h$ is equivalent to $h$. In this work, we consider the widely used Taylor-Hood conforming finite-element spaces $\HDisph = \mathcal P_{k+1}(\mathcal T_h)^2 \cap \HDisp $ and $\Hph = \mathcal P_{k}(\mathcal T_h) \cap \Hp$, where $\mathcal P_k(\mathcal T_h)$ denotes space of the continuous piecewise polynomials of degree $k$. \fixme{  Nonconforming see ...}
The discrete counterpart to \eqref{twofields} reads
\begin{subequations}\label{twofields_h}
\begin{align}\label{twofields_h1}
% ToDo BC
%(\sigmaexp{\Disp_h}- \alpha p_h  \bI,\nabla \DispTest)
(\symgrad{\Disp_h}{\DispTest})+(\lambda(\div \Disp_h) \bI- \alpha p_h  \bI,\nabla \DispTest)
  =
( \bff,\DispTest) \\
 (s_0 p_h,q)+(\alpha \div \Disp_h, q)+(\kappa \nabla p_h,\nabla q) = (g,q)\label{twofields_h2}
\end{align}\end{subequations}
%there exists two constants $\rho_1$ and $\rho_2$ such that for the diameter $\rho(T)$ of each element $T\in \mathcal T_h$ it holds $h\rho_1\leq \rho(T) \rho_1
Recall that then, neither the approximation of the elastic stress 
$$ \Stress_h := \sigmaexp{\Disp_h}$$ nor the approximation of the Darcy Velocity $$\psi_h := - \kappa \nabla p_{h}$$
are $\Hdiv$-conforming, such that in particular the evaluation of the surface tension forces is not possible. The aim of this paper is to present different reconstructions in the $\Hdiv$-conforming spaces \begin{align}
RT_k(\mathcal T_h) = \fixme{...}
\end{align}

\begin{thm}[A posteriori estimate for the two-fields formulation]
\begin{align}
\energy{(\Disp,p)}^2 = 
\energy{(\Disp,p)}^2 \leq \eta(\Disp_h,p_h) 
\end{align}
\end{thm}
\begin{proof}
From the variational formulations  we have
\begin{align*}
\energy{(\Disperror,p_F-p_h)}^2  &= \energyds{2}{\Disperror}{p_F-p_h} \\&= 
a((\Disperror,p_F-p_h),(\Disperror,p_F-p_h)) 
\end{align*}
and for all $(\DispTest,q)$
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))    = & 
\atwo{\Disperror}{\DispTest}{(p_F-p_h)}{}\\&
+\atwo{\Disperror}{}{(p_F-p_h)}{q}
\end{align*}
Inserting $\psi =-\kappa \nabla p_F$, $\psi_h =-\kappa \nabla p_h$, $\TotalStress = \TotalStressdef{}{} $ 
and $\TotalStress_h = \TotalStressdef{\Disp_h}{p_h} $,
we obtain
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))  =& 
(\TotalStress-\TotalStress_h,\symgrad{\DispTest}{})
-(\psi-\psi_h,\nabla q)\\
&+s_0(p_F-p_h,q)+\alpha(\div(\Disperror),q)
\end{align*}
Since $\TotalStress$ and $\TotalStress_h$ are symmetric, integration by parts together with ? leads to 
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))   &= 
(\div \left(\TotalStress-\TotalStress_h\right),{\DispTest}{})
+(\div \left(\psi-\psi_h \right), q)\\
&-(\div \psi,q) + (g,q)-s_0(p_h,q)-\alpha(\div \Disp_h,q) \\
=&
(\bff,{\DispTest}{})
-(\div \TotalStress_h,{\DispTest}{})
-(\div \psi_h, q)+ (g-s_0p_h-\alpha\div \Disp_h,q) \\
=&
(\bff-\Pi^k \bff,{\DispTest}{})
+ (\div \left(\TotalStress_h^R-\TotalStress_h\right),{\DispTest}{})
+( \psi_h^R-\psi_h, \nabla q)\\
%&+ (g,q)-s_0(p_h,q)-\alpha(\div \Disp_h,q)-
%\left(\Pi^{k-1}(g-s_0(p_h,q)-\alpha(\div \Disp_h),q\right)\\
&+\left((id - \Pi^{k-1}) \left( g-s_0p_h-\alpha\div \Disp_h\right),q\right)
\end{align*}
\fixme{Are they some superconvergence property that we could use here in the g oscillation? }
Fisrt term is oscillation term, with a local constant since for any rigid body motion
\begin{align*}
(\bff-\Pi^k \bff,{\DispTest}{}) 
=
\sumT
(\bff-\Pi^k \bff,{\DispTest}{}-\rho)
\leq
C_{K,T} \norm{\bff-\Pi^k \bff} \norm{\symgrad{\DispTest}{}}
\end{align*}
Similary for fourth term using local Poincaré.
\begin{align*}
\fixme{\text{add details}}
\end{align*}
Second term: use Lemma \ref{vertex-patch-all}
\begin{align*}
 (\div \left(\TotalStress_h^R-\TotalStress_h\right),{\DispTest}{})
 & = 
 \fixme{check sign}
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\nabla {\DispTest}{})
\\
 & = 
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\symgrad{\DispTest}{})
  +
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\as{\DispTest}{})  
  \\
 & = 
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\symgrad{\DispTest}{})   
  +
  ( \TotalStress_h^R,\as{\DispTest}{}) \\
  & \leq 
  \norm{\sym (\TotalStress_h^R-\TotalStress_h)}\norm{\symgrad{\DispTest}{}}
  + 
C_K    \norm{\as \TotalStress_h^\Delta}
\norm{\symgrad{\DispTest}{}}
\end{align*}
The third term can be handled by Cauchy Schwarz.
\end{proof}
\fixme{Efficiency ? }

==> old_2.tex <==
\section{Stress and Flux variables in the Biot Model}

on a reference configuration $\Omega\subset \R^2$
For $\bx \in \Omega$ and at a time $t$, the fluid pressure is denoted by $\phi(\bx,t)$ and the displacement of the solid by $\Disp(\bx,t)$. 


\fixme{In this section, we should emphase the importance of the auxiliary variables like stress and flux and their physical meanings!}
The classical Biot model of consolidation under our consideration describes a linearly elastic and porous structure with reference configuration $\Omega\subset \R^2$, which is saturated by a slightly compressible viscous fluid. For $\bx \in \Omega$ and at a time $t$, the fluid pressure is denoted by $\phi(\bx,t)$ and the displacement of the solid by $\Disp(\bx,t)$. 

$\Omega$ is assumed to be a an open, bounded, and connected domain with Lipschitz-continuous boundary $\Gamma$ divided in two disjoint nonempty subsets $\Gamma_u$ and $\Gamma_p$. On $\Gamma_u$, homogeneous displacement boundary conditions are imposed while surface traction forces are prescribed on $\Gamma_p$.
The equations for the quasi-static Biot model are given by 
\begin{subequations}\label{Biot}\begin{align}
\div \left(
	\sigmaexp{\Dispt}- \alpha \phi(t)  \bI
 \right)  = \bff(t) \\
 s_0 \difft \phi(t)+\alpha \div \difft \Dispt-\div(\kappa \nabla \phi(t)) = g(t)
\end{align}\end{subequations}
The analysis of numerical treatment can be reduced to stationary case \fixme{(this sentence needs to be rewriten in a more diplomatic way)}
\begin{subequations}\label{Biot_stationary}\begin{align}
\div \left(
	\sigmaexp{\Disp}- \alpha \phi  \bI
 \right)  = \bff \\
 s_0 \phi+\alpha \div  \Disp-\div(\kappa \nabla \phi) = g
\end{align}\end{subequations}
where for simplicity we did not change the definition of $\bff$ and $g$. Note that the first equation is the momentum equation and can be rewritten as 
\begin{align}
\div \left(
	\Stress(\Disp) - \alpha \phi  \bI
 \right)  = \bff
 \end{align}
 where $\Stress(\Disp) := \sigmaexp{\Disp}$ denotes the elastic stress or 
 \begin{align*}
\div 
	\TotalStress 
  = \bff \ ,
 \end{align*} 
 with the total stress tensor $\TotalStress = \TotalStressdef{}{}$. %expressing the fact that an increase in pore pressure induces a dilation of the matrix in response to the added stress.
  \fixme{point out the importance of Hdiv conformity for those variables. Conservation law. Surface tension forces of the solid structure}

\fixme{emphize the advantages of RT reconstructions and cite papers with AW reconstructions.}
\fixme{make clear that the motivation is two-folds: approximation in Hdiv and a posteriori}
For the fluid velocity, the Braess-Schöberl algorithm rom \cite{BraSch:08} reconstructing the conforming approximation of the solution of the Poisson equation in the Raviart-Thomas Finite element space can be used. A major advantage is that the reconstruction can be localised on the vertex-patches
\begin{equation}
  \omega_\nu := \bigcup \{ T \in \cT_h : \nu \mbox{ is a vertex of } T \} \: .
  \label{eq:vertex_patch}
\end{equation}
involving the partition of unity
\begin{equation}
  1 \equiv \sum_{\nu \in \mathcal V_h} \chi_\nu  ,
  \label{eq:partition_of_unity_1}
\end{equation}
and the localised broken Raviart-Thomas spaces
\begin{align}
RT^\Delta_\nu := \{ 
\bw_h
 \in  L^2(\omega_\nu)  : \left.
 \bw_h 
 \right|_T 
 \in RT_k (T), \bw_h \cdot \bn = 0 \} \ .
\end{align}
To a function $f \in L^2(\Omega)$ and a flux $\bw_h \in \mathbb P_k(\mathcal T_h)^2$ we denotes the Braess-Schöberl reconstruction of order $k$ by $\bw_h^R = \BR^k(f, \bw_h )$ the function 
$\bw_h^R \in RT^k(\mathcal T_h)$  with 
$\bw_h^R = \bw_h +\bw_h^{\Delta}$ and 
$\bw_h^{\Delta} = \sum_{\nu \in \mathcal V} \bw_{h,\nu}^{\Delta}$
and $\bw_{h,\nu}^{\Delta} \in DRT^\Delta(\omega_\nu)$ such that $\|\bw_{h,\nu}^{\Delta}\|$ is
minimized subject to the following constraints:
\begin{equation}
  \begin{split}
     \div \: {\bw_{h,\nu}^\Delta } 
    & = - \Pi^k_T \left( ({\bff} + \div \: \bw_h) \phi_\nu \right) \text{ on each }T\in \omega_\nu
   \\
     \llbracket \bw_{h,\nu}^\Delta \cdot \bn \rrbracket_S 
    & =  - \Pi^{k}_S  \left( \phi_\nu \llbracket 
    \bw_h \cdot \bn 
    \rrbracket_S \right) \text{ for each } S \text{ interior edge in } \omega_z \ .
  \end{split} 
  \label{eq:equilibration_conditions_local}
\end{equation}
To simplify the notation, we define
$\BR^k_\nu(f, \bw_h ) := \bw_{h,\nu}^\Delta$ 
\fixme{( Can i write this inverse mapping in an explicit way? )}
and for a tensor $\Stress = 
\left( \Stress_1 \ \Stress_2 \right)^\top \in RT^k(\mathcal T_h)^2$ and a vector-valued function $\bff = 
\left( f_1 \ f_2 \right)^\top \in L^2(\Omega)^2$ , the Braess-Schöberl construction $\BR^k(f, \bw_h )$ is defined elementwise:
\begin{align}
\BR^k(\bff, \Stress ) := 
\begin{pmatrix}
 \BR^k(f_1, \Stress_1 ) \\
 \BR^k(f_2, \Stress_2 )
\end{pmatrix}
\end{align}

For the purpose of the exposition, we recall the condition for existence and the properties of the Braess-Schöberl construction in the next theorem. 
\begin{thm}[Braess-Schöberl algorithm for Poisson equation, \cite{}]
Assume that $f \in \mathbb P _{k-1}(\mathcal T_h)$ and $\tilde p_h \in \mathcal P _k(\mathcal T_h) \cap H_{\Gamma_u}^1(\Omega) $ is the discrete solution of the Poisson equation, i.e.
\begin{align}
\left ( \nabla \tilde p_h, \nabla q \right) = \left ( f,  q \right) \quad \forall q \in \mathcal P _k(\mathcal T_h) \cap H_{\Gamma_u}^1(\Omega)  \ .
\end{align}
The Braess-Schöberl reconstruction $\bw_h^R = \Psi(f, \bw_h) \in RT{k-1}(\tri)$ exists and satisfies
\begin{subequations}
\begin{align}
\div \bw_h^R &= f \\
\norm{\nabla (\tilde p-\tilde p_h)} &\leq \norm{\bw_h^R-\bw_h} \\
\fixme{\text{insert other properties i may need}}
\end{align}
\end{subequations}
where $\tilde p$ denotes the exact solution of the Poisson equation $\div \nabla \tilde p = - f$.
\end{thm}
Note that a crucial condition for this theorem to hold is the compatibility condition
\begin{align*}
\fixme{\text{insert compatibility condition}}
\end{align*} 
In order to apply this construction to the Biot problem, we shift the first two terms of \eqref{twofields_h2} to the right side, following \cite{Riedelbeck} and define $\tilde g = g- s_0 p_h-\alpha \div \Disp $.


For the reconstruction of the stress, \cite{BerKobMolSta:19} showed that the symmetry has to be taken into account. The authors considered a the displacement pressure formulation but we will show that the reconstruction can be applied to the standard conforming displacement formulation of linear elasticity. In fact, the construction of the authors is equivalent to a minimization in the divergence free Raviart-Thomas space of order $k$
 \begin{align}
RT_k^\times(\omega_\nu) = 
\left\{
\bw \in RT_k(\omega_\nu) \ : \ \div \bw = 0
 \right\} \ ,
\end{align} 
where the difference between the reconstructed stress and the stress computed from the variational formulation belong to the 
weakly symmetric broken Raviart-Thomas space of order $k$
 \begin{align*}
DRT_k^{ws}(\omega_\nu) = 
\left\{
\begin{pmatrix}
 \tau_1
 \\ 
 \tau_2
 \end{pmatrix}
 \in (DRT_k(\omega_\nu))^2 \ : 
  \right.%&
 %\\ & 
 \left.
\left(
\tau_1 \cdot 
 \begin{pmatrix} 1 \\ 0 
 \end{pmatrix}
 -
  \tau_2 \cdot 
 \begin{pmatrix} 0 \\ 1  
 \end{pmatrix}, \chi
 \right)_{\omega_\nu}
  = 0 
  \text{ for all }\chi \in \mathcal P^k(\mathcal T_h)
 \right\} \ .
\end{align*}
%For $\Stress_\nu \in DRT_k(\omega_\nu)^2$, let $\symcomp{\nu}{ \Stress_\nu}$ denotes the minimisation of the norm under the symmetry constraint:
%\begin{align}
%\symcomp{\nu}{ \Stress_\nu}
% = \argmin_{
% \underset{s.t.\ \Stress_\nu + \Stress \in RT_k^{ws}(\omega_\nu) }{
% \Stress \in RT_k^\times(\omega_\nu)^2}
% } \|\Stress_\nu + \Stress \|
%\end{align}
For $\Stress_h \in DRT_k(\tri)^2$, let $\symcomp{\nu}{ \Stress_\nu}$ denotes the minimisation of the norm under the symmetry constraint:
\begin{align}
\symcomp{\nu}{ \Stress_h}
 =  \argmin_{
 \underset{s.t.\ \Stress_h + \Stress \in DRT_k^{ws}(\omega_\nu) }{
 \Stress \in RT_k^\times(\omega_\nu)^2}
 } \|\Stress_h + \Stress \|
\end{align}
Further notation:
\begin{align}
\symcomp{}{\Stress_h} := \sum\limits_{\nu\in \nodes} \symcomp{\nu}{ \Stress_h} \text{ and }\widetilde \Pi(\Stress_h):=\Stress_h + \symcomp{}{\Stress_h} 
\end{align}
\fixme{this is a projection on a $\sigma$-dependant space, maybe the notation should be changed.}

\begin{thm}
Assume that ${\bff} \in (\mathbb P _k(\mathcal T_h))^2$. Let $\tilde \Disp_h \in \HDisph$ be the discrete solution of the variational formulation
\begin{align} \label{standard_conforming_elasticity}
 \left( \Stress({\tilde\Disp_h}), \symgrad{\DispTest}{} \right) = \left( {\bff} , \DispTest \right)
 \quad \forall \DispTest \in \HDisph \ .
\end{align}
Then, the weakly symmetric reconstruction 
$\Stress_h^R({\tilde\Disp_h}) =
 \widetilde \Pi \left(
\BR^k ({\bff}, \Stress({\tilde\Disp_h})) \right)		$
exists and satisfies
\begin{subequations}
\begin{align}
\div \Stress_h^R({\tilde\Disp_h}) = {\bff}\\
\fixme{\text{In particular here we should list all the properties for elasticity}}
\end{align}
\end{subequations}
\end{thm}
\begin{proof}
\fixme{...}
\end{proof}



\begin{remark}
enough degrees of freedom since the Braess-Schöberl reconstruction already satisfies the weekly symmetric condition.
\end{remark}

\mynote{
Set $\Stress_{h,z}^\Delta = \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta$
\begin{align*}
( \div \: \Stress_{h,z}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}
    & = - ( ( \bff + \div \: \Stress_h ) \phi_z ,
    \bz_{h,z}  )_{\omega_z,h}
    \\
    \langle \llbracket \Stress_{h,z}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            = & - \langle \llbracket \Stress_h \cdot \bn \rrbracket_S \, \phi_z , \zeta \rangle_S
   \\
    (
     \Stress_{h,z}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & = 0
\end{align*}
Since $\Stress_{h,z,BR}^\Delta$ satisfies the first two equations
it remains\\
$( \div \: (\Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta) , 
\bz_{h,z} )_{\omega_z^\ast,h}
     = - ( ( \bff + \div \: \Stress_h ) \phi_z ,
    \bz_{h,z}  )_{\omega_z,h}$\\
    i.e.
    $( \div \: 
\Stress_{h,z,AS}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}  = 0$\\
und $\langle \llbracket \Stress_{h,z,AS}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            =  0$
       also minimize $\| \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta \|$
       \begin{align*}
( \div \: \Stress_{h,z,AS}^\Delta , 
\bz_{h,z} )_{\omega_z^\ast,h}
    & =0
    \\
    \langle \llbracket \Stress_{h,z}^\Delta \cdot \bn \rrbracket_S , \zeta \rangle_S
            = & 0
   \\
    (
     \Stress_{h,z,AS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & =  -\Stress_{h,z,BS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} 
\end{align*}
Find $\Stress_{h,z,AS}^\Delta$ in RTdivfree, such that 
$\| \Stress_{h,z,BR}^\Delta +
\Stress_{h,z,AS}^\Delta \|$ is minimum, and
       \begin{align*}
    (
     \Stress_{h,z,AS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} & =  -(\Stress_{h,z,BS}^\Delta ,
     J^d (\gamma_{h,z}) 
    )_{\omega_z} 
\end{align*}
}


Energy-norm:
\begin{align}
\energy{(\Disp,p)}^2 = \energyds{2}{\Disp}{p}
\end{align}
Error estimator
\begin{align}
\eta(\Disp_h,p_h) = \left( \norm{(\Stress_h^R}^2
+
\norm{\kappa \bw_h^R}^2
\right)^{\frac 1 2}
\end{align}
more general version of Vertex-patch estimate.
\begin{lem}
\label{vertex-patch-all}
Let $\Stress_h \in DRT_k(\tri) $. 
If it exists, the reconstruction 
$\widetilde \Pi  {\BR^k({\bff}, \Stress_h ) }$ satisfies 
\begin{align}
 (\as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },{\DispTest}{})
 \leq  C_K \| \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h )  }\|
 \norm{\symgrad{\DispTest}{}}
\end{align}
for any $\DispTest  \in \HDisp$, where $C_K$ depends only on the shape regularity of the triangulation $\tri$.
\end{lem}
\begin{proof}
For any $\nu \in \nodes$, the existence of $ \widetilde \Pi  {\BR^k({\bff}, \Stress_h )} $ implies that we can find $\symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )}}
 \in RT_k^\times(\omega_\nu)^2$ with 
\begin{align*}
{\BR^k({\bff}, \Stress_h )}  
+ \symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )} } \in DRT_k^{ws}(\omega_\nu) 
\end{align*}
such that for all $\chi \in \mathcal P^k(\tri)$
\begin{align*}
\left(\as
\widetilde \Pi  {\BR^k({\bff}, \Stress_h )} 
, \chi 
\right) 
=
 \sum\limits_{\nu \in \mathcal V_h}
\left(\as
{\BR^k({\bff}, \Stress_h )}  
+ \symcomp{\nu}{ {\BR^k({\bff}, \Stress_h )} }
, \chi 
\right)_{\omega_\nu}
= 0
\end{align*}
 holds. In particular, for any rigid body motion $\brho$
 \begin{align*}
\left(\as
\widetilde \Pi  {\BR^k({\bff}, \Stress_h )} 
, \nabla\brho
\right) 
= 0
\end{align*}
 such that we can use the Korn inequality to obtain
\begin{align*}
 (\as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },{\DispTest}{})
 &= 
  \left(
  \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h ) },
{\DispTest-\brho}
\right) \leq C_K 
\| \as \widetilde \Pi  {\BR^k({\bff}, \Stress_h )}\| 
\norm{\symgrad{\DispTest}{}}
\end{align*}
involving a local Korn constant $C_K$ depending only on the shape triangularity of the triangulation $\tri$.
%  \begin{equation}
%    \begin{split}
%      | ( \bas \: \bsigma_h^R , \bnabla (\bu - \bu_h) ) |
%      & = | ( \bas \: \bsigma_h^R , \sum_{z \in \cV_h} \left( \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \right) \phi_z ) | \\
%      & = \left| \sum_{z \in \cV_h} ( \bas \: \bsigma_h^R ,
%      \left( \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \right) \phi_z )_{\omega_z} \right| \\
%      & = \left| \sum_{z \in \cV_h} ( (\bas \: \bsigma_h^R) \phi_z , \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) )_{\omega_z} \right| \\
%      & \leq \sum_{z \in \cV_h} \| (\bas \: \bsigma_h^R) \phi_z \|_{\omega_z}
%      \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z} \\
%      & \leq \sum_{z \in \cV_h} \| \bas \: \bsigma_h^R \|_{\omega_z} \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z} \: .
%    \end{split}
%    \label{eq:asym_partition}
%  \end{equation}
%  For all rigid body modes $\brho \in \bR\bM$, $\bnabla \brho = \bJ^d (\balpha_z)$ holds with some $\balpha_z \in \R^{d (d-1)/2}$
%  and therefore
%  \begin{equation}
%    \inf_{\balpha_z} \| \bnabla (\bu - \bu_h) - \bJ^d (\balpha_z) \|_{\omega_z}
%    \leq \inf_{\brho \in \bR\bM} \| \bnabla (\bu - \bu_h - \brho) \|_{\omega_z}
%    \leq C_{K,z} \| \bepsilon (\bu - \bu_h) \|_{\omega_z}
%    \label{eq:Korn_average}
%  \end{equation}
\end{proof}


\section{Three field formulation}
$p := - \lambda \div \Disp + \alpha \phi$ introduced in  \cite{Lee} . 

$p_S = \lambda \div \Disp = \alpha \phi -p_T$

\begin{equation}
\begin{aligned}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \boldsymbol{H}_{0}^{1} \\
%
-\left(\div \Disp, q\right)
-\left(\lambda^{-1} p, q\right)
+\left(\alpha \lambda^{-1} \phi, q\right) 
&=0, & \forall \quad q \in L^{2} \\
%
\left(\alpha \lambda^{-1} p, \psi\right)-2\left(\alpha^{2} \lambda^{-1} \phi, \psi\right)-\left(\kappa \nabla \phi, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in H_{0}^{1} 
\end{aligned}\end{equation}

Our purpose is a robust a posteriori error estimate, when $\lambda$ tends to infinity.
Note that in the incompressible case, the equations are decoupled which reflect the physical process.
\begin{equation}
\label{Lee}
\begin{aligned}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \boldsymbol{H}_{0}^{1} \\
%
-\left(\div \Disp, q\right)
&=0, & \forall \quad q \in L^{2} \\
%
-\left(\kappa \nabla \phi, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in H_{0}^{1} 
\end{aligned}\end{equation}

\begin{equation}
\label{Lee_h}
\begin{aligned}
\symgrad{\Disp_h}{\DispTest} 
-\left(\div \DispTest, p_{T,h}\right) 
&=(\bff, \DispTest), 
& \forall \quad \DispTest \in \HDisph \\
%
-\left(\div \Disp, q\right)
&=0, & \forall \quad q \in \Hp \\
%
-\left(\kappa \nabla p_{F,h}, \nabla \psi\right) 
&=\left(g, \psi\right), & \forall \quad \psi \in \HDisph 
\end{aligned}\end{equation}

We now return back to a general $\lambda$, possibliy infinity.
\begin{equation}
  \Stress (\Disp,p) = 2 \mu \symgrad{\Disp}{} + p\bI
  \label{eq:direct_stress}
\end{equation}
The approximation
\begin{equation}
  \Stress_h (\Disp_h,p_h) = 2 \mu \symgrad{\Disp_h}{} + p_{h} \bI
  \label{eq:direct_stress_processing}
\end{equation}

First line:
\begin{align*}
\symgrad{\Disp}{\DispTest} 
-\left(\div \DispTest, p\right) 
&=
\symgrad{\Disp}{\DispTest} 
+\left(\div \DispTest,  p_S - \alpha \phi\right) \\&
=
\left(
\Stress(\Disp),
\symgrad{\DispTest}{} 
\right)
-\left(\div \DispTest,  \alpha \phi\right) 
\end{align*}

For the reconstruction of an $\Hdiv$-conforming stress tensor we use the main result from \cite{BB} about the weakly symmetric stress reconstruction of the displacement-pressure formulation. We recall this result here for the purpose of the exposition.
\begin{thm}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor arising from displacement-pressure formulation]
\label{thm-weaklystressreco}
 \fixme{Write it here, maybe in a more general way?}
\end{thm}

\begin{cor}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor for the three-field formulation of the Biot model]
 \fixme{...}
\end{cor}
\begin{proof}
\fixme{ compatibility condition}
\end{proof}

As for the two-fields formulation, we will reconstruct the total stress tensor. In this three fields formulation, the approximation of the stress tensor reads
\begin{align*}
\TotalStress_h = \TotalStressdef{\Disp_h,p_{S,h}}{p_{F,h}}
\end{align*}
From \eqref{} and \eqref{} we therefore obtain the equilibration condition 
 \begin{align*}
\div 
	\TotalStress 
  = \bff \ .
 \end{align*} 
 
\begin{thm}[\cite{BB}  Weakly symmetric reconstruction of the stress tensor arising from displacement-pressure formulation]
 \fixme{Write it here, maybe in a more general way?}
\end{thm}
\begin{proof}
\fixme{ Use \ref{thm-weaklystressreco}}
\end{proof}

\begin{cor}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. $p_h$ is the discrete solution of the Poisson equation with right hand side $\tilde f =  {\Pi_k(g- s_0 p_h-\alpha \div \Disp_h )}$ and its Braess-Schöberl reconstruction $\bw_h^R$ 
exists and satisfies
\begin{equation}
  \begin{split}
     \div \: {\bw_{h}^R } 
    & =  {\Pi^{k-1}(g- s_0 \phi_h-\alpha \div \Disp_h )}  
  \end{split}
\end{equation}
\begin{align*}
\fixme{...}
\end{align*}
\end{cor}
\begin{proof}
The crucial compatibility condition holds, since $p_h$ is the solution of the Poisson equation with right hand side $f =  {\Pi_k(g- s_0 p_h-\alpha \div \Disp_h )}$.
\end{proof}
This leads to a $\Hdiv$ conforming reconstruction which can be used to evaluate the surface traction forces as illustrated in the numerical experiments in section \ref{sec-numerical-results}.

\begin{cor}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. The reconstruction 
\begin{align}
\Stress_h^R =\widetilde \Pi {\BR^k({\bff}-\nabla p_h, \Stress({\Disp_h})) }
\end{align}
exists and satisfies
\begin{subequations}
\begin{align}
\Stress_h^R &\in \bHdiv \\
\div\Stress_h^R &= \Pi^k \bff -\nabla p_h\\
\norm{\Stress - \Stress_h^R}_{\Gamma_u, div} &\leq h^k | \Stress|_{k+1} \fixme{\text{add oscillations and u,p norm?}}
\end{align}
\end{subequations}
\end{cor}
The reconstruction of $\Stress$ allows for the evaluation of the surface traction force, see {\fixme{example X}}. For the a posteriori error estimation however, it is necessary to consider the reconstruction of the total stress reconstruction, as presented in the following theorem.

\begin{thm}
Let $(\Disp_h,p_h)$ be the solution of the two-fields formulation \eqref{twofields_h}. The reconstruction 
\begin{align}
\TotalStress_h^R 
=\widetilde \Pi{\BR^k_\nu({\bff}, \TotalStress_h ) }
\end{align}
exists and satisfies
\begin{align*}
\TotalStress_h^R \in (\bHdiv)^2\\
\div \TotalStress_h^R  = \Pi^k \bff \\
\end{align*} 
\end{thm}
\begin{proof}
The construction of $\TotalStress_h^R$ implies that
$\TotalStress_h^R = \TotalStress_h +\TotalStress_h^{\Delta}$ with
$\TotalStress_h^{\Delta} = \sum_{\nu \in \mathcal V} \TotalStress_{h,\nu}^{\Delta}$
and $\TotalStress_{h,\nu}^{\Delta} \in (DRT^\Delta(\omega_\nu))^2$ such that $\|\TotalStress_{h,\nu}^{\Delta}\|$ is
minimized subject to the following constraints:
\begin{equation}
  \begin{split}
     \div \: {\TotalStress_{h,\nu}^\Delta } 
    & = -  {\Pi^k \left(\phi_\nu\left(g- s_0 p_h-\alpha \div \Disp_h
    - \div \: \bpsi_h  \right)\right)} 
 \\
     \llbracket \bpsi_{h,\nu}^\Delta \cdot \bn \rrbracket_S 
    & =  - \Pi^{k}_S \left( \phi_\nu  \llbracket \bpsi_h \cdot \bn  \rrbracket_S\right) \text{ for each } S \text{ interior edge in } \omega_z
  \end{split}
\end{equation}
\end{proof}

\section{Compressible case and two-fields formulation}
The two-fields formulation \fixme{insert citations} seeks $(\Disp,p_F) \in \HDisp \times \Hp$ such that
\begin{subequations}\label{twofields}
\begin{align}
%(\sigmaexp{\Disp}- \alpha p_F  \bI,\nabla \DispTest)
(\symgrad{\Disp}{\DispTest})+(\lambda(\div \Disp) \bI- \alpha p_F  \bI,\nabla \DispTest)
  &=
( \bff,\DispTest) \quad \forall \DispTest \in \HDisp\\
 (s_0 p_F,q)+(\alpha \div \Disp, q)+(\kappa \nabla p_F,\nabla q) &= (g,q) \quad \forall q \in \Hp
\end{align}\end{subequations}
holds for all $(\DispTest,q) \in \HDisp \times \Hp$.
For the finite element approximation of the system \eqref{Biot_stationary}, the saddle-point problem \eqref{twofields} is solved in finite-element spaces. To this end, let $\mathcal T_h$ be a regular triangulation of the domain $\Omega$ where the diameter $\rho(T)$ of each element $T\in \mathcal T_h$ is equivalent to $h$. In this work, we consider the widely used Taylor-Hood conforming finite-element spaces $\HDisph = \mathcal P_{k+1}(\mathcal T_h)^2 \cap \HDisp $ and $\Hph = \mathcal P_{k}(\mathcal T_h) \cap \Hp$, where $\mathcal P_k(\mathcal T_h)$ denotes space of the continuous piecewise polynomials of degree $k$. \fixme{  Nonconforming see ...}
The discrete counterpart to \eqref{twofields} reads
\begin{subequations}\label{twofields_h}
\begin{align}\label{twofields_h1}
% ToDo BC
%(\sigmaexp{\Disp_h}- \alpha p_h  \bI,\nabla \DispTest)
(\symgrad{\Disp_h}{\DispTest})+(\lambda(\div \Disp_h) \bI- \alpha p_h  \bI,\nabla \DispTest)
  =
( \bff,\DispTest) \\
 (s_0 p_h,q)+(\alpha \div \Disp_h, q)+(\kappa \nabla p_h,\nabla q) = (g,q)\label{twofields_h2}
\end{align}\end{subequations}
%there exists two constants $\rho_1$ and $\rho_2$ such that for the diameter $\rho(T)$ of each element $T\in \mathcal T_h$ it holds $h\rho_1\leq \rho(T) \rho_1
Recall that then, neither the approximation of the elastic stress 
$$ \Stress_h := \sigmaexp{\Disp_h}$$ nor the approximation of the Darcy Velocity $$\psi_h := - \kappa \nabla p_{h}$$
are $\Hdiv$-conforming, such that in particular the evaluation of the surface tension forces is not possible. The aim of this paper is to present different reconstructions in the $\Hdiv$-conforming spaces \begin{align}
RT_k(\mathcal T_h) = \fixme{...}
\end{align}

\begin{thm}[A posteriori estimate for the two-fields formulation]
\begin{align}
\energy{(\Disp,p)}^2 = 
\energy{(\Disp,p)}^2 \leq \eta(\Disp_h,p_h) 
\end{align}
\end{thm}
\begin{proof}
From the variational formulations  we have
\begin{align*}
\energy{(\Disperror,p_F-p_h)}^2  &= \energyds{2}{\Disperror}{p_F-p_h} \\&= 
a((\Disperror,p_F-p_h),(\Disperror,p_F-p_h)) 
\end{align*}
and for all $(\DispTest,q)$
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))    = & 
\atwo{\Disperror}{\DispTest}{(p_F-p_h)}{}\\&
+\atwo{\Disperror}{}{(p_F-p_h)}{q}
\end{align*}
Inserting $\psi =-\kappa \nabla p_F$, $\psi_h =-\kappa \nabla p_h$, $\TotalStress = \TotalStressdef{}{} $ 
and $\TotalStress_h = \TotalStressdef{\Disp_h}{p_h} $,
we obtain
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))  =& 
(\TotalStress-\TotalStress_h,\symgrad{\DispTest}{})
-(\psi-\psi_h,\nabla q)\\
&+s_0(p_F-p_h,q)+\alpha(\div(\Disperror),q)
\end{align*}
Since $\TotalStress$ and $\TotalStress_h$ are symmetric, integration by parts together with ? leads to 
\begin{align*}
a((\Disperror,p_F-p_h),(\DispTest,q))   &= 
(\div \left(\TotalStress-\TotalStress_h\right),{\DispTest}{})
+(\div \left(\psi-\psi_h \right), q)\\
&-(\div \psi,q) + (g,q)-s_0(p_h,q)-\alpha(\div \Disp_h,q) \\
=&
(\bff,{\DispTest}{})
-(\div \TotalStress_h,{\DispTest}{})
-(\div \psi_h, q)+ (g-s_0p_h-\alpha\div \Disp_h,q) \\
=&
(\bff-\Pi^k \bff,{\DispTest}{})
+ (\div \left(\TotalStress_h^R-\TotalStress_h\right),{\DispTest}{})
+( \psi_h^R-\psi_h, \nabla q)\\
%&+ (g,q)-s_0(p_h,q)-\alpha(\div \Disp_h,q)-
%\left(\Pi^{k-1}(g-s_0(p_h,q)-\alpha(\div \Disp_h),q\right)\\
&+\left((id - \Pi^{k-1}) \left( g-s_0p_h-\alpha\div \Disp_h\right),q\right)
\end{align*}
\fixme{Are they some superconvergence property that we could use here in the g oscillation? }
Fisrt term is oscillation term, with a local constant since for any rigid body motion
\begin{align*}
(\bff-\Pi^k \bff,{\DispTest}{}) 
=
\sumT
(\bff-\Pi^k \bff,{\DispTest}{}-\rho)
\leq
C_{K,T} \norm{\bff-\Pi^k \bff} \norm{\symgrad{\DispTest}{}}
\end{align*}
Similary for fourth term using local Poincaré.
\begin{align*}
\fixme{\text{add details}}
\end{align*}
Second term: use Lemma \ref{vertex-patch-all}
\begin{align*}
 (\div \left(\TotalStress_h^R-\TotalStress_h\right),{\DispTest}{})
 & = 
 \fixme{check sign}
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\nabla {\DispTest}{})
\\
 & = 
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\symgrad{\DispTest}{})
  +
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\as{\DispTest}{})  
  \\
 & = 
  ( \left(\TotalStress_h^R-\TotalStress_h\right),\symgrad{\DispTest}{})   
  +
  ( \TotalStress_h^R,\as{\DispTest}{}) \\
  & \leq 
  \norm{\sym (\TotalStress_h^R-\TotalStress_h)}\norm{\symgrad{\DispTest}{}}
  + 
C_K    \norm{\as \TotalStress_h^\Delta}
\norm{\symgrad{\DispTest}{}}
\end{align*}
The third term can be handled by Cauchy Schwarz.
\end{proof}
\fixme{Efficiency ? }
